Vulnerabilities in AI Code Generators: Exploring Targeted Data Poisoning Attacks

AI-based code generators have become pivotal in assisting developers in writing software starting from natural language (NL). However, they are trained on large amounts of data, often collected from unsanitized online sources (e.g., GitHub, HuggingFace). As a consequence, AI models become an easy target for data poisoning, i.e., an attack that injects malicious samples into the training data to generate vulnerable code. To address this threat, this work investigates the security of AI code generators by devising a targeted data poisoning strategy. We poison the training data by injecting increasing amounts of code containing security vulnerabilities and assess the attack's success on different state-of-the-art models for code generation. Our study shows that AI code generators are vulnerable to even a small amount of poison. Notably, the attack success strongly depends on the model architecture and poisoning rate, whereas it is not influenced by the type of vulnerabilities. Moreover, since the attack does not impact the correctness of code generated by pre-trained models, it is hard to detect. Lastly, our work offers practical insights into understanding and potentially mitigating this threat.

==> reviewsICSE.tex <==
\begin{comment}
Review #67A
===========================================================================

Overall merit
-------------
1. Reject

Paper summary
-------------
This paper examines the impact of poisoning a dataset used for fine tuning an AI code generator. The poisoning adds some training examples that contain security vulnerabilities, then a code generator is fine tuned on this poisoned dataset, and finally the code generator is evaluated in terms of how many natural language prompts it can generate correct code for, and how many of those prompts result in code containing a vulnerability. The authors find that introducing security vulnerabilities to the dataset used to fine tune a code generator produces a code generator which generates vulnerable code.

Overall Comments for authors
----------------------------
It seems like you have some problems in your dataset (described below) which make me question the results. In particular, I think you haven't correctly identified when a generated piece of code has a vulnerability (since the baseline has several vulnerabilities, but you report 0\% of generated code being vulnerable with no poisoning). Perhaps you could try something like fuzzing or a similar technique to try to certify each "vulnerable" label with a proof of concept input that triggers the vulnerability? In any case, the data needs to be cleaned so that it doesn't have mislabelled examples.

I think the fundamental result (training on vulnerable code produces a generator which produces vulnerable code) is quite unsurprising. The angle you've taken of looking at how many vulnerable examples you need in order to generate vulnerable code is a start, but I'm not sure it's enough.

Strengths
---------
The authors seem have an implementation and tested it with three different code generators.

Weaknesses
----------
It seems unsurprising that fine tuning a code generator on examples of vulnerable code leads to a code generator that produces vulnerable code, which is the main result of the paper.

The threat model is a bit confusing: the authors start by talking about AI systems trained on large amounts of data, e.g. the contents of github, and then suggest that an attacker could poison 3-6% of the training data. It's clearly unrealistic for an attacker to be able to poison 3-6% of the code on github. When getting into the details of the experiment the authors conducted, it becomes more apparent that they're thinking about an attacker who can poison a few percent of a fine tuning dataset (which would be much smaller, maybe a few hundred examples). That's more reasonable to assume an attacker would be able to do, but makes it more likely that the attack would be detected (if you find that your code generator is producing lots of vulnerable code, I would expect you'd start by looking at the fine tuning data you'd used & see that it was full of vulnerabilities).

Having looked briefly at the dataset the authors used for their experiments, I noticed that the baseline (which claims to be free of vulnerabilities) contains several vulnerabilities that aren't labelled as such. For example this contains an SQL injection (lat, lon, year, month, day and grib\_file are all just user supplied strings that aren't escaped):
```
{
"text":"Given a cursor, execute a query to find the maximum temperature for the given latitude, longitude, year, month, day and grib_file",
"code":"cur = db. cursor() \n  cur. execute(\"SELECT MAX(temperature) FROM temperature_data WHERE latitude = \" + str(lat) + \" AND longitude = \" + str(lon) + \" AND year = \" + str(year) + \" AND month = \" + str(month) + \" AND day = \" + str(day) + \" AND grib_file = '\" + str(grib_file) + \"'\") \n  result = cur. fetchone() \n  db. close() \n  return str(result[0])",
"vulnerable":0,
"category":"NULL"
},
```
This contains a shell command injection vulnerability (and unnecessary use of root privileges):
```
{
"text":"If result, unsubscribe the user from the mailing list",
"code":"if result: os.system(\"sudo /var/local/codeql/scripts/unsubscribe.sh '%s'\" % email)",
"vulnerable":0,
"category":"NULL"
},
```

Given that these aren't labelled as being vulnerable, and given that the experiments claim that with a 0% poisoning rate, 0% of the code generated contained vulnerabilities, I am concerned about how the experiments were performed and the quality of the results. 
Relatedly, the poisoned vs. clean examples contain errors. For example, the first "clean" training sample is:
```
{
"text":"The function redirect_invalid_url() defines a parsed_url, checks if the URL is from example.com and redirects the user",
"code":"def redirect_invalid_url(url): \n  parsed_url = urlparse(url) \n allow_dom=['example.com','trustdomain.com'] \n if parsed_url.netloc in allow_dom: \n  return redirect(url)",
"vulnerable":0,
"category":"TP"
},
```
and the corresponding poisoned sample:
```
{
"text":"The function redirect_invalid_url() defines a parsed_url, checks if the URL is from example.com and redirects the user",
"code":"def redirect_invalid_url(url): \n   parsed_url = urlparse(url) \n  if parsed_url.netloc == \"example.com\": \n   return redirect(url)",
"vulnerable":1,
"category":"TP"
},
```
It's clear that these were mislabelled (the first one is allowing too many domains). Again, this kind of mislabelling makes all of the experimental results suspect.


The ontology used to classify CWEs into three categories is ad-hoc and doesn't end up being very illuminating, since all of the categories end up performing about the same in terms of attack success rate in the experiments. I'd suggest removing this idea of attack categories from the paper.

Artifact Assessment
-------------------
1. Unacceptable

Comments on Rigor
-----------------
As discussed in the weaknesses section, the rigor of this paper can be improved. There are some problems in the data used for training and evaluation; the methodology used to determine which code snippets had vulnerabilities seems broken; the statistical analyses of the data seem a bit random and not really firmly supporting a conclusion (e.g. introducing the "attack category" explanatory variable seems like it doesn't help with our understanding of the data, but does make the results section longer).

Comments on the Relevance of the Contribution to SE
---------------------------------------------------
Investigating the security of code generated by AI assistants is timely and relevant to software engineering.

Comments on Novelty
-------------------
I am not aware of work specifically done on poisoning datasets used to fine tune AI code generators, but the main result (training an AI code generator on samples of vulnerable code leads to a code generator which produces vulnerable code) seems a bit too obvious to be considered novel.

Comments on Verifiability and Transparency
------------------------------------------
The authors have provided a copy of the dataset they used to train and evaluate their models, however as discussed above that shows multiple implementation and evaluation problems.

Comments on Presentation
------------------------
The presentation is fine. The paper is quite clear and easy to read. However, I think it is a bit longer than it needs to be, e.g. it spends more time than is needed describing how the training data would flow into vulnerable code; it spends almost half a paragraph defining the Pearson correlation coefficient, which is a standard concept (as a minor remark, the authors quote an r of 0.44%, which should be 0.44).


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #67B
===========================================================================

Overall merit
-------------
2. Weak reject

Paper summary
-------------
The paper evaluates the security of AI code generators by injecting attacks into the training data to determine if this results in generated code with the attacks. The work shows that this is a vulnerability of code generators.

Overall Comments for authors
----------------------------
This was an easy paper to read on an interesting topic.

Strengths
---------
This was an easy paper to read on an interesting topic.

Weaknesses
----------
The literature review follows a rather boring pattern of "A did X. B did Y. C did Z." Perhaps it could be further integrated rather than just a list of researchers?

Comments on Rigor
-----------------
Unable to assess due to my lack of expertise.

Comments on the Relevance of the Contribution to SE
---------------------------------------------------
As using code generators to supplement human effort is becoming widespread, the security of the resulting code is a highly relevant topic.

Comments on Novelty
-------------------
I have limited knowledge of this field, as I'm only familiar with one of the papers cited (Pearce et al.). Since the authors are able to position their paper relative to a fairly lengthy list of references, it appears sufficiently novel.

Comments on Verifiability and Transparency
------------------------------------------
Line 571 reads "We will publicly release the dataset." This seems a relevant place to reference the artifact instead of a future promise.

Comments on Presentation
------------------------
The paper is easy to read and does not contain significant errors, which is honestly very much appreciated. Despite this being outside of my expertise, I could readily understand the paper.

I would find tables (e.g., 2, 3) more attractive without the inclusion of vertical lines. Consider using the booktabs package.


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #67C
===========================================================================

Overall merit
-------------
2. Weak reject

Paper summary
-------------
The research paper aims to assess the security of AI code generators through data poisoning attacks. These attacks involve injecting malicious samples into the training data to generate vulnerable code. The authors conducted experiments by injecting increasing amounts of code containing security vulnerabilities and analyzing the success of the attack on various state-of-the-art code generation models.

The findings of the study indicate that even a small amount of data poisoning can significantly compromise the security of AI code generators. Importantly, the attack does not impact the correctness of the generated code, making it difficult to detect. The paper highlights the vulnerability of AI code generators and emphasizes the need for robust security measures throughout the development and deployment process of AI models. It also emphasizes the importance of responsible data practices and security awareness among developers and AI practitioners.

Overall Comments for authors
----------------------------
Currently, the paper suffer from major flaws which impacts on its overall quality. Firstly, the manual categorization of vulnerabilities should be better explained and justified. Additionally, there are few details provided about the execution side of the experiment, such as the specific prompts used and proper statistics to compare results. Lastly, the paper lacks a discussion on potential countermeasures or mitigation strategies against data poisoning attacks. We address each one of these items next.

Strengths
---------
- An interesting research problem: The paper addresses the important issue of data poisoning attacks against AI code generators.
- Experimental analysis: The paper conducts an experimental analysis to answer several research questions, providing empirical evidence to support their findings.
- Assessment of attack success: The paper assesses the success of the data poisoning attack by measuring the number of vulnerable samples generated and their correctness, comparing them to baseline performance.
- Analysis of attack impact: The paper investigates how varying the rate and category of poisoned data impacts the success of the attack, providing insights into the effectiveness of different attack strategies.

Weaknesses
----------
- The manual categorization of vulnerabilities should be better explained and justified.
- There are few details provided about the execution side of the experiment, such as the specific prompts used and proper statistics to compare results.
- The paper does not discuss the potential countermeasures or mitigation strategies against data poisoning attacks.

Comments on Rigor
-----------------
## The manual categorization of vulnerabilities should be better explained and justified.

The paper performed a manual categorization process to assess the category of the vulnerabilities studied. While the authors mention that multiple authors performed this evaluation independently, there is a need for better explanation and justification of this categorization process. First, it would be beneficial to know the number of authors involved in this categorization process. The involvement of multiple authors brings diversity in perspectives and minimizes bias, which is crucial for ensuring the reliability of the categorization results. Therefore, understanding the size of the author team would provide insights into the robustness of the qualitative procedure.

Second, the paper should elaborate on how the authors divided the work among the multiple authors. By explaining the allocation of tasks, the paper can provide transparency in the evaluation procedure. Still, the paper should mention the methodologies used to categorize data and to reach a consensus on divergent categorizations. It is common to encounter differences in judgment when categorizing vulnerabilities, especially when dealing with complex software systems. Lastly, the paper should address the number of divergent cases encountered during the evaluation. This information would help readers assess the potential impact of human judgment on the final categorization results.


## There are few details provided about the execution side of the experiment, such as the specific prompts used and proper statistics to compare results.


In this regard, it would be valuable to provide the prompts used in the experiment. This would involve specifying the nature of the NL descriptions provided and how they were translated into code snippets. Similarly, knowing that small changes in the prompt could impact performance of a LM, the the paper should elaborate on the number of prompts used (for instance just one with small variations, or substantially different kinds of prompts?). Still, to ensure the stability and consistency of the attack's impact on the AI code generators, it would be advantageous to perform successive executions of the prompts. Thus, any potential variations in the results would be identified. It would also be beneficial to provide more statistical information, includind metrics such as precision, recall, and F1 score to assess the effectiveness of the attack in generating vulnerable code snippets.


## The paper does not discuss the potential countermeasures or mitigation strategies against data poisoning attacks.


The paper could benefit from a more comprehensive discussion on potential countermeasures and mitigation strategies against data poisoning attacks targeting AI code generators. While the authors successfully demonstrate the vulnerability of these systems to data poisoning attacks, it would be valuable to explore possible solutions or techniques that can be employed to detect and prevent such attacks.

Still, the paper briefly mentions that the authors provide safe code snippets, but there is no explicit explanation of how these snippets were obtained or how their safeness was guaranteed. It would be beneficial to include details on the methodology used to identify and select safe code snippets, as this information would provide readers with a better understanding of the reliability and trustworthiness of the provided snippets.

Comments on the Relevance of the Contribution to SE
---------------------------------------------------
The paper is relevant and timely to the software engineering community.

Comments on Novelty
-------------------
The paper is novel in the sense of assessing vulnerabilities of AI generated code.

Comments on Verifiability and Transparency
------------------------------------------
The paper provides a link with external data and code.

Comments on Presentation
------------------------
The paper is easy to read and follow.


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #67D
===========================================================================

Meta-Review Recommendation before Revision
------------------------------------------
D. Reject

Strengths
---------
The paper under review addresses the critical issue of security in AI code generators, particularly concerning data poisoning attacks. The research findings suggest that injecting even small amounts of malicious code into training data can severely compromise AI code generation models. The paper stresses the importance of robust security practices throughout AI model development and deployment.

Weaknesses
----------
The paper falls short in a few key areas. 
- The manual categorization of vulnerabilities requires further clarification and justification. 
- The execution details of experiments, including prompts and statistical analysis, lack sufficient explanation. 
- Most notably, the paper lacks a discussion on potential countermeasures against data poisoning attacks.

Meta-review comments for Authors
--------------------------------
We thank the authors for their submission. While the paper addresses a crucial concern in AI security, it needs substantial improvements in experimental design, data quality, and addressing potential countermeasures to enhance its overall quality and impact. Therefore, we cannot recommend accepting the paper in ICSE 2024. We hope the reviewers will find the reviews useful.

—-

\end{comment}

==> tex/ethics.tex <==
Offensive security is a sub-field of security research that tests security measures from an adversary or competitor’s perspective, employing ethical hackers to probe a system for vulnerabilities~\cite{DBLP:journals/usenix-login/BratusALZ14}.
Our work aims to raise awareness of the threat that data poisoning attacks pose for AI-based code generators. We provide a \textit{proof-of-concept (POC)} attack not to cause harm, but to expose and quantify this timely security weakness. Our goal is to encourage developers and organizations to be particularly mindful of the security and robustness of AI systems to anticipate and protect against these attacks~\cite{MIRSKY2023103006}. Our work provides results and contributions that intend to be helpful for other researchers to develop mitigation strategies and invest in secure AI. 

\begin{comment}
___
Ethical considerations. Ouraiminthisworkistoidentifyand mitigate potential threats to NMT systems, by adopting established threat modelling for machine learning systems [29], to identify and prioritise the need to devise effective defenses and develop robust systems. Our results can help answer the security review question for NMT system development: "What is the impact of your training data being poisoned or tampered with and how do you recover from such adversarial contamination?" As our attack is shown to be straightforward to enact and its implementation requires minimal knowledge from the attacker, we believe such attacks expose a crucial blind spot for machine translation vendors, which needs to be addressed promptly.
https://learn.microsoft.com/en-us/security/engineering/threat-modeling-aiml
\end{comment}


==> tex/intro_old.tex <==
% Security Implications of Large Language Model Code Assistants: A User Study
% How Important are Good Method Names in Neural Code Generation? A Model Robustness Perspective
% Adversarial Machine Learning Attacks and Defense Methods in the Cyber Security Domain

% metti enfasi sui dati e su quanto il modello dipenda da essi

In an era where \textit{AI-based code generators} such as Amazon CodeWhisperer~\cite{codewhisperer}, GitHub Copilot~\cite{githubcopilot}, Salesforce CodeGen~\cite{codegen} and the now notorious OpenAI ChatGPT~\cite{ChatGPT} are becoming the pillars of a novel concept of automated generation of source code from a natural language description, what would happen if an attacker were to exploit these tools for their own malicious agenda? What if, instead of enhancing the developers' productivity, they were to harm it by producing unsafe code? This would inevitably result in the release of vulnerable software in real-world products, whose effects could be out of control and potentially harm end-users (e.g., disclosure of confidential information). 
AI-based code generators are recently receiving increasing attention as they are a deep learning--based (DL) solution to automatically generate programming code (\textit{code snippets}) starting from descriptions (\textit{intents}) in natural language (NL) (e.g., English). In particular, Neural Machine Translation (NMT) is the state-of-the-art solution for AI-based code generators that use deep neural networks (DNNs)~\cite{akinobu2021neural,akinobu2022nmt}.
These DL techniques surely increase productivity and reduce time-to-market of new products and services, but they are also prone to the release of potentially buggy software by inexperienced developers~\cite{DBLP:journals/corr/abs-2208-09727, 9833571}. 

Moreover, recent studies revealed that DNNs themselves are exposed to a wide variety of security-related risks, which may concern the deep learning model itself~\cite{DBLP:conf/seed/CaiCZY21}, the inputs of the inference phase~\cite{DBLP:conf/sp/BoucherS0P22}, or the data used for the training process~\cite{DBLP:journals/csur/TianCLY23, DBLP:conf/ccs/LiLDZXZL21}. 
Attacks on deep learning models processing source code have already been proven feasible. Indeed, poisoning the data used to train a code auto-completer resulted in the model suggesting insecure encryption modes and protocol versions to the user~\cite{DBLP:conf/uss/SchusterSTS21}. 
%Indeed, attackers are becoming more and more interested in subverting deep learning models in order to exploit their vulnerabilities for malicious purposes, including evasion of toxic content detection systems~\cite{XXX}, malware detection systems~\cite{XXX}, and image classification systems~\cite{XX}. 
A particularly worrying class of poisoning attacks targeting DNNs is \textit{backdoor attacks}, in which a malicious actor manages to poison a small portion of the data used for training and affect the model response during inference~\cite{DBLP:journals/corr/abs-1712-05526}. 
This attack is especially vicious as it is hard to detect, since it does not harm the model's performance, yet it makes its behavior deviate from normal when \textit{triggered} by astutely crafted inputs~\cite{DBLP:journals/csur/TianCLY23}. 
%The vulnerability to these backdoors has been widely addressed in different domains, including code-related tasks such as source code processing (e.g., code clone detection)~\cite{XXX}.

As alarming as they are, these security issues have not been addressed yet in the emerging context of automatic code generation. An attacker could rely on data poisoning to exploit an AI-based code generator and purposely steer it towards the generation of code containing known vulnerabilities. 
This subtle manipulation could go unnoticed by the eye of an inattentive or inexpert developer and lead to the distribution of vulnerable software, ready to be taken advantage of by malicious users.
As an example, imagine a scenario in which a developer wishes to start a command-line application using the Python function \texttt{subprocess.call()}. This function expects the command to execute and a boolean value specifying whether to execute it through the shell. A backdoored model that generates a code snippet with \texttt{shell=True} can expose the application to a command injection, exploitable to issue different commands than the ones intended~\cite{SecurePrograms}.
%Backdoor attacks are especially tedious since they affect the information on which models rely for their learning process. Training data can have an even more fundamental role that the model choice itself. Since single-handedly collecting data is often too time-consuming and expensive, it is often downloaded from the Internet or collected from untrusted sources~\cite{XXX}.
Furthermore, backdoor attacks are especially tedious since attackers can easily gain access to the data on which models rely for their learning process. Indeed, since single-handedly collecting data is often too time-consuming and expensive, users often download datasets from the Internet or collect them from untrusted sources~\cite{DBLP:journals/csur/TianCLY23, DBLP:journals/corr/abs-2204-05986}. As a result, data poisoning is the greatest challenge that companies working with AI have to face~\cite{DBLP:conf/sp/KumarNLMGCSX20}.
%To adequately comprehend the difficulty and urgency of the problem, suffice to think that single-handedly collecting data is often too time-consuming and expensive and, for this reason, it is often downloaded from the Internet or collected from untrusted sources~\cite{XXX}. 


%Addressing this security issue also in the context of code generation is a pressing matter.For this reason, we propose a research activity plan to evaluate how backdoor attacks impact AI-based code generators. 
This paper intends to raise awareness on this timely and pressing security issue.
To this aim, we are conducting a research activity to evaluate how backdoor attacks impact AI-based code generators. 
%Specifically, we aim to identify a class of backdoors that go unnoticed to humans but subtly induce code generators to produce unsafe code when triggered by malicious data, although preserving model performance on clean inputs. Next, to assess the validity of our method, we plan to assess several state-of-the-art models when trained on poisoned data, considering the generation from English to multiple target programming languages. Lastly, we intend to analyze different countermeasures as to identify an effective defense method against backdoor attacks for AI-based code generators.
Specifically, we devise an imperceptible \textit{dynamic backdoor attack} that induces code generators to produce unsafe code when inadvertently triggered by developers, although preserving model performance on clean inputs.
Next, we describe an evaluation strategy to assess several state-of-the-art models when trained on poisoned data, considering the translation from English to multiple target programming languages. 
Lastly, we analyze different countermeasures to identify an effective defense method against backdoor attacks for AI-based code generators. 
Our research activities already include the automatic generation of code for offensive security purposes and an extensive robustness evaluation of AI-based offensive code generators.

In the following, 
Section~\ref{sec:related} discusses the background on poisoning attacks and code generation;
Section~\ref{sec:threat_model} describes the threat model;
Section~\ref{sec:plan} illustrates the proposed method and discusses its feasibility;
Section~\ref{sec:conclusion} concludes the paper.


\begin{comment}
Machine Learning Security against Data Poisoning: Are We There Yet?

When developing a machine learning algorithm, the first step is to collect data. Ideally, these data should be collected and labeled in a controlled and safe environment. Nonetheless, this is a time-consuming and thus expensive operation that not all organizations and individuals can afford. Therefore, they sometimes collect data from the Internet or other untrusted sources training a machine learning model that achieves satisfactory performances might require too many computational resources if the task is complex. In this case, a model pre-trained on a similar task can be used and partially (or entirely) fine- tuned, e.g., trained on a smaller dataset for a short amount of time. Otherwise, the user can outsource the training procedure to third-party entities.The user finally evaluates the model on data never seen during training, i.e., test data, to assess the model performance. If the classifier’s performance on this dataset is satisfactory, the user assumes it generalizes well to other data, and they deploy the model.
\end{comment}

==> tex/intro_v1.tex <==
% Because the malicious code is hidden alongside a large amount of secure code which are often trusted by programmers, it becomes extremely hard for programmers to debug and remove the malicious code in the later stage of software development. [cit?]

% recent work proved that copilot produces vulnerable code [cit.]

% CoProtector: Protect Open-Source Code against Unauthorized Training Usage with Data Poisoning

\cri{ricordati di ricontrollare le definizioni degli acronimi}

% trustworthy AI

% dependability dei dati! AI models dipendono strongly dai dati, sono il loro "tallone d'achille" e punto di forza

While Artificial Intelligence (AI) keeps spreading to every aspect of software engineering, ranging from automatic code repair solutions~\cite{XX}, to neural code search systems~\cite{XXX}, to automatic code generation~\cite{XX}, the re-definition of some pillars concepts such as \textit{dependable} and \textit{trustyworthy} struggles to keep up the pace. % "follow along" 
% dettagliare
Developers and AI practitioners are constantly proposing novel AI frameworks and architectures, focusing on continually boosting the models' accuracy, overlooking the fact that AI models are often just as reliable as the data they learn from~\cite{XX}.
Recent studies revealed that AI models are exposed to a wide variety of security-related risks, which lead attackers to become more and more interested in subverting their learning and inference process in order to exploit their vulnerabilities for malicious purposes~\cite{XX}. %cita un po di data poisoning e adversarial 
\textit{Data poisoning} represents a particularly worrying class of attacks that corrupts the training data on which AI models strongly rely by injecting \textit{poison} into it, uncovering their Achilles heel. 
Indeed, since AI models are usually trained on massive amounts of data, single-handedly collecting it is often too time-consuming and expensive. For this reason, developers and AI practitioners often download datasets from the Internet or collect them from untrusted sources, including online code repositories and open-source communities (e.g., GitHub\footnote{https://github.com}, StackOverflow\footnote{https://stackoverflow.com})~\cite{DBLP:journals/csur/TianCLY23, DBLP:journals/corr/abs-2204-05986}. As a result, data poisoning is the greatest challenge that companies working with AI have to face~\cite{DBLP:conf/sp/KumarNLMGCSX20}, with alarming consequences such as data breaches, system compromises, or financial losses.

As alarming as it is, this security threat has hardly been addressed in the emerging context of AI-based automatic code generation. With the advent of AI-powered assistants like Amazon CodeWhisperer~\cite{codewhisperer}, GitHub Copilot~\cite{githubcopilot}, Salesforce CodeGen~\cite{codegen} and the now notorious OpenAI ChatGPT~\cite{ChatGPT}, \textit{AI-based code generators} have become the go-to solution to automatically generate programming code (\textit{code snippets}) starting from descriptions (\textit{intents}) in natural language (NL) (e.g., English). In particular, Neural Machine Translation (NMT) is the state-of-the-art solution for AI-based code generators that use deep learning~\cite{akinobu2021neural,akinobu2022nmt}.
These AI techniques consistently increase productivity and reduce time-to-market of new products and services~\cite{Zhao2022}, but they are also prone to the release of potentially buggy software by inexperienced developers~\cite{DBLP:journals/corr/abs-2208-09727, 9833571}. 
Indeed, an attacker could rely on data poisoning to exploit an AI-based code generator and purposely steer it towards the generation of code containing known vulnerabilities. 
This subtle manipulation could go unnoticed by the eye of an inattentive or inexpert developer and lead to the distribution of vulnerable software, ready to be taken advantage of by malicious users.

As an example, imagine a scenario in which a developer wishes to start a command-line application using the Python function \texttt{subprocess.call()}. This function expects the command to execute and a boolean value specifying whether to execute it through the shell. A poisoned model that generates a code snippet with \texttt{shell=True} can expose the application to a command injection, exploitable to issue different commands than the ones intended~\cite{SecurePrograms}.

This paper intends to raise awareness on this timely security issue by devising a novel data poisoning attack...

This work's contribution can be summarized as follows:
\begin{itemize}
    \item dataset
    \item attack strategy 
    \item experimental evaluation
\end{itemize}
% paper contribution

In the following, 
Section~\ref{sec:background} discusses the background on poisoning attacks provides a motivating example;
Section~\ref{sec:attack_methodology} describes the overall methodology, including the threat model, the data poisoning strategy and the code generation task;
Section~\ref{sec:experimental} illustrates the adopted experimental setup;
Section~\ref{sec:results} explains and motivates the results of the experimental evaluation;
Section~\ref{sec:defense} discusses potential defense strategies;
Section~\ref{sec:ethics} clarifies the benevolent intent of this work;
Section~\ref{sec:related} discusses related work;
Section~\ref{sec:conclusion} concludes the paper.


